TroVE: Inducing Verifiable and Efficient Toolboxes for Solving Programmatic Tasks

Language models (LMs) can solve tasks such as answering questions about tables or images by writing programs. However, using primitive functions often leads to verbose and error-prone programs, and higher-level functions require expert design. To enable better solutions without human labor, we ask code LMs to curate reusable high-level functions, and use them to write solutions. We present TROVE, a training-free method of inducing a verifiable and efficient toolbox of functions, by generating via using, growing, and periodically trimming the toolbox. On 11 datasets from math, table question answering, and image reasoning tasks, TROVE consistently yields simpler solutions with higher accuracy than baselines using CODELLAMA and previous methods using GPT, while using 79-98% smaller toolboxes. TROVE further enables 31% faster and 13% more accurate human verification than baselines. With the same pipeline, it creates diverse functions for varied tasks and datasets, providing insights into their individual characteristics.

==> appendices/d_optimal-ordering.tex <==
\section{Exploring Optimal Ordering}
\label{app:d:optimal-ordering}

We have shown that \textsc{TroVE} is robust to randomized ordering. We further investigate if a potentially optimal ordering exists that yields the best performance.

We hypothesize that an optimal ordering clusters examples using the same function. To get example clustering information, we take the results from running \textsc{TroVE}, and group together examples that use the same function in their solutions. We rank function clusters from the highest usage frequency to the lowest, to prioritize major function categories. We order examples in each cluster by their original order in the dataset. If an example uses multiple functions, we only include it in the last appearing function cluster, to ensure all functions required (should be) available. We denote this as \textit{post-hoc}.
\dfcomment{It's not too clear to me why this would be the optimal ordering. Is Trove more likely to use recently induced rather than older functions? If not, why is it helpful to have sequences of examples that all use the same function?}

\begin{table}[ht]
\small 
\centering 
\resizebox{0.45\textwidth}{!}{
    \begin{tabular}{l|r|r|r}
    \toprule
    \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{Evaluation Metrics}} \\
    {} & \multicolumn{1}{c|}{acc $\uparrow$} & \multicolumn{1}{c|}{\# ops $\downarrow$} & \multicolumn{1}{c}{\# lib $\downarrow$} \\
    \midrule
    \multicolumn{4}{c}{\hlcell MATH$_{algebra}$} \\
    \midrule
    {original} & {0.25} & {18.8} & {10} \\
    {post-hoc} & {0.26} & {19.0} & {10} \\
    \midrule
    \multicolumn{4}{c}{\hlcell HiTab} \\
    \midrule
    {original} & {0.18} & {9.3} & {5} \\
    {post-hoc} & {0.17} & {9.0} & {10} \\
    \midrule
    \multicolumn{4}{c}{\hlcell \textsc{GQA}} \\
    \midrule
    {original} & {0.43} & {20.6} & {6} \\
    {post-hoc} & {0.46} & {20.1} & {8} \\
    \bottomrule
    \end{tabular}
}
\vspace{-1mm}
\caption{\textsc{CodeLLaMa} results with post-hoc ordering.}
\vspace{-1mm}
\label{tab:optimal-ordering}
\end{table}

From \autoref{tab:optimal-ordering}, post-hoc example ordering slightly improves on three datasets, however, not comprehensively on all metrics. In MATH$_{algebra}$, accuracy increases by $+ 1\%$ but at the cost of $+ 0.2$ more operations. In Hitab, although accuracy drops by $- 2\%$, but it saves operation counts by $- 0.3$. In GQA, both accuracy ($+ 3\%$) and complexity ($- 0.5$) scores better, but at the cost of 2 more functions.
